Symbolic tensor calculus on manifolds: a SageMath implementation

These lecture notes present a method for symbolic tensor calculus that (i) runs on fully specified smooth manifolds (described by an atlas), (ii) is not limited to a single coordinate chart or vector frame, (iii) runs even on non-parallelizable manifolds and (iv) is independent of the symbolic backend used to perform calculus at the level of coordinate expressions. In addition to the main ideas, we discuss some details of the implementation in the open-source mathematics software system SageMath, which has been performed via the SageManifolds project.

==> CCIRM-pagedegarde.tex <==
\thispagestyle{empty}
\addtocounter{page}{-2}
\enlargethispage{2cm}
\begingroup
\pagecolor{fond}
\frenchspacing
\def\UrlFont{\sffamily\color[gray]{.4}}
\url@sfstyle
\DeclareRobustCommand*{\staburl}{\hyper@normalise\staburl@}
\def\staburl@#1{\hyper@linkurl{\color{blue}\Hurl{#1}}{#1}}
\parindent0pt
\strut\kern-6mm\raisebox{-35mm}[0pt][0pt]{\includegraphics[width=4cm]{logo-cirm}}\\*[4.5cm]
\begin{center}
\color{textecouv}
\ifx\cdr@conftitle@french\@empty\else
{\Huge \itshape \cdr@conftitle@french\\[24pt]}\fi
\ifx\cdr@resps\@empty\else
\begin{otherlanguage}{french}\def\@@and{et}%
  \textsc{Rencontre organis\'ee par :}\\
  \Large \cdr@resps
\end{otherlanguage}
\\[18pt]\fi
\currentmonth\ \currentyear
\end{center}

\vspace*{2.5cm}

\begin{flushleft}
  \begingroup
  \author@andify\authors
  {\large\ignorespaces\authors\unskip}%
  \\[4pt]
  \begin{hyphenrules}{nohyphenation}%
    \def\\{\allowbreak}
    \textbf{\ignorespaces\@title\unskip}\par
  \end{hyphenrules}
  \endgroup
\end{flushleft}
\normalsize
\ifx\currentvolume\@empty\else
Vol.~\currentvolume\fi\ifx\currentissue\@empty\else,
\no\currentissue\fi\
(\currentyear), \ifnum\c@article>\z@ \Coursname\ \no\TheExp, \fi
p.~\cdr@start@page-\cdr@end@page.\\[6pt]
\normalsize%\sf
<\staburl{\journalURL item?id=\CDRidart}> \vfill
\begin{center}
{\Large
Centre international de rencontres math\'ematiques\\
\large
U.M.S. 822 C.N.R.S./S.M.F.\\
Luminy (Marseille) \textsc{France}\\[2pt]}
\vskip0pt plus.4fill
\href{\CDRbaseURL}{\includegraphics{logocedram}}\\
 \small{\usefont{T1}{ptm}{m}{it}Texte mis en ligne dans le cadre du\\
  Centre de diffusion des revues acad\'emiques de math\'ematiques}\\
\url{\CDRbaseURL}\\[10mm]
\end{center}
\endgroup
%\pagebreak
\cleardoublepage
\endinput

